EventGround: Narrative Reasoning by Grounding to Eventuality-centric Knowledge Graphs

Narrative reasoning relies on the understanding of eventualities in story contexts, which requires a wealth of background world knowledge. To help machines leverage such knowledge, existing solutions can be categorized into two groups. Some focus on implicitly modeling eventuality knowledge by pretraining language models (LMs) with eventuality-aware objectives. However, this approach breaks down knowledge structures and lacks interpretability. Others explicitly collect world knowledge of eventualities into structured eventuality-centric knowledge graphs (KGs). However, existing research on leveraging these knowledge sources for free-texts is limited. In this work, we propose an initial comprehensive framework called EventGround, which aims to tackle the problem of grounding free-texts to eventuality-centric KGs for contextualized narrative reasoning. We identify two critical problems in this direction: the event representation and sparsity problems. We provide simple yet effective parsing and partial information extraction methods to tackle these problems. Experimental results demonstrate that our approach consistently outperforms baseline models when combined with graph neural network (GNN) or large language model (LLM) based graph reasoning models. Our framework, incorporating grounded knowledge, achieves state-of-the-art performance while providing interpretable evidence.

==> sections/background.tex <==
\section{Background}
\label{sec:background}

A narrative is a series of related events that can happen everywhere in our daily life.
Understanding and reasoning based on narratives is a fundamental task~\cite{mostafazadeh2016corpus,li2018constructing,mori2020finding} and has attracted much interest in the NLP community since it is related to downstream applications like text summarization and dialogue generation.

The most crucial problem in narrative reasoning is modeling the relationship between events, which often requires commonsense knowledge~\cite{mostafazadeh2016corpus}. 
Many large scale commonsense knowledge graphs (KGs) such as ATOMIC~\cite{sap2019atomic}, ConceptNet~\cite{speer2017conceptnet}, ASER~\cite{zhang2020aser,zhang2022aser} and GLUCOSE~\cite{mostafazadeh2020glucose} have been constructed in recent years.
How to leverage the commonsense-rich knowledge in these resources remains a problem.
Current solutions can be coarsely categorized into two groups: the knowledge model paradigm and the retrieval-and-integration paradigm.
Figure~\ref{fig:paradigm} gives an overview of the two paradigms.
Here the sample question is from Story Cloze Test~\cite{mostafazadeh2016corpus} and the eventuality\footnote{In this work, we use the term ``eventuality'', which includes abstract events, states and activities~\cite{zhang2022aser}, to distinguish from specific events.} subgraph is from ASER.

\begin{figure*}[t]
\centering
\vspace{-10pt}
\includegraphics[width=1\textwidth]{figs/ParadigmComparison.pdf}
\vspace{-10pt}
\caption{Overview of the knowledge model paradigm (left) and the retrieval-and-integration paradigm (right). The knowledge model paradigm fine-tunes PLMs with eventuality knowledge and then makes predictions through the fine-tuned blackbox knowledge model. The retrieval-and-integration paradigm retrieves relevant subgraphs of the story context and then makes predictions according to the retrieved subgraph.}
\vspace{-10pt}
\label{fig:paradigm}
\end{figure*}

The knowledge model paradigm leverages external KGs by feeding knowledge pieces (usually in the form of triplets) into pretrained language models (PLMs) and fine-tuning the PLMs with carefully designed training objectives~\cite{yu2020cocolm,zhou2021modeling}.
The fine-tuned knowledge model can then compute a probability based on the narrative sequence to perform inference.
{\color{red}
However, there is a gap between piecemeal training and inference of the entire sequence.
}
% Although the fine-tuned knowledge models can remember the knowledge pieces, it is difficult for the models to understand the entire KG with the graph structure broken down.
Besides, as a common weakness of PLMs, knowledge models suffer from the poor interpretability where they cannot offer explainable evidence at any steps.

On the other hand, the retrieval-and-integration paradigm leverages external KGs by retrieving knowledge relevant to the input texts and integrating the retrieved knowledge into prediction models.
With the retrieved knowledge, the prediction models can provide evidence along with the predictions.
However, early works in the retrieval-and-integration paradigm focus on entity-centric KGs~\cite{zhang2019ernie,liu2020k}, which has small semantic coverage in narrative reasoning tasks. 
\citet{lv2020integrating} first propose to leverage ASER in the script reasoning task~\cite{li2018constructing}, in which the event texts constructed from event tuples, removing complexities in real-world free texts.
Even so, the semantic matching algorithm in this work often fails in retrieval or introduces noisy knowledge.

% In this work, we extend the retrieval-and-integration paradigm to perform high quality knowledge retrieval and interpretable reasoning on free text based narrative reasoning tasks. 
The wide adoption of AI critically needs explainability~\cite{hoffman2018metrics}. Thus, despite the appeal of a simpler pipeline (aided by the availability of large PLMs), this work focus on improving retrieval-and-integration approach.
For high quality knowledge retrieval, we propose an event acquisition pipeline including event extraction, normalization, and abstraction to mine multi-granularity events from input free texts with the help of semantic parsing.
With the acquired multi-granularity events, we use semantic matching models to ground the events to relevant eventualities in KGs, and thus construct a joint subgraph containing both events from input texts and the eventualities from KGs.
Then, we encode the subgraph with graph neural networks (GNNs) to make prediction. 
The constructed subgraph as well as the GNN parameters can provide interpretable evidence.
% Note that we still leverage PLMs for text embedding, but they are constrained in interpretable prediction, thus not used to compute the subgraph probability.
% As a result, our approach doesn't critically rely on large PLMs.

==> sections/old_introduction.tex <==
\section{Introduction}


% {\color{orange}
%  Background here. 
%  why not entity linking but event linking?
% }
% Events are regarded as one of the primitive semantic units in many NLP research works \cite{zhang2020aser, yu2020cocolm, zhong2022unsupervised, zhang2022aser}. 

%write by Jacky
Narrative reasoning, specifically story ending prediction and script reasoning tasks, required more ability and knowledge than narrative comprehension ability. \{comment:cite some paper to show different knowledge help narrative reasoning task\}. Since the narrative is meaningfully connected by the semiotic representation of a sequence of events ~\cite{ryan2007toward,onega2014narratology}, it also required the ability to understand relations between events from the narrative. \{comment: Start to describe the story/idea (adopt what knowledge for these task)\} For example, consider the following narrative sentence:
\begin{quote}
\vspace{-6pt}
\textit{``They arrived and learned from the news that it was a terrible storm.''}
\vspace{-6pt}
\end{quote}
This narrative sentence can be broken down into multiple sub-sentences (regarded as an \textit{event}).
\begin{quote}
\vspace{-6pt}
\textit{(\textbf{E1}) They arrived. (\textbf{E2}) They learned from the news (that it was a terrible storm). (\textbf{E3}) It was a terrible storm.}
\vspace{-6pt}
\end{quote}
where each \textit{event} consists of a verb and one or more arguments. These events, which are seen as \textit{basic semantic units} in many NLP research \cite{zhang2020aser, yu2020cocolm, zhong2022unsupervised, zhang2022aser}, express majority and core meaning from the narrative context.

In fact, apart from the event comprehension ability, the narrative reasoning process also reliance on the background world knowledge (e.g. commonsense knowledge) \cite{day1998extensive}. Given a sentence ``\textit{the firefighters are rushing into a burning house},'' by utilizing the background world knowledge, human can infer that there is a fire and probably a fire engine nearby, and then may reason that the firefighters are trying to rescue someone in the house.





Understanding narratives requires the understanding of events.
Consider the following sentence:
\begin{quote}
\vspace{-6pt}
``They arrived and learned from the news that it was a terrible storm.''
\vspace{-6pt}
\end{quote}
It can be broken down into multiple sub-sentences:
\begin{quote}
\vspace{-6pt}
(\textbf{E1}) They arrived. (\textbf{E2}) They learned from the news (that it was a terrible storm). (\textbf{E3}) It was a terrible storm.
\vspace{-6pt}
\end{quote}
where each of them can be regarded as an \textit{event} with a verb and one to several arguments.
These events, which are seen as \textit{basic semantic units} in many NLP research \cite{zhang2020aser, yu2020cocolm, zhong2022unsupervised, zhang2022aser}, express most of the meaning in the context.


% https://www.thoughtco.com/world-knowledge-language-studies-1692508
Apart from the event knowledge in contexts, the comprehension of narratives also depends on our background world knowledge \cite{day1998extensive}.
% In addition to the context itself, understanding narratives requires complex knowledge.
For example, when given ``\textit{the firefighters are rushing into a burning house},'' we can infer that there is a fire and there is probably a fire engine nearby.
We may also reason that the firefighters are trying to rescue someone in the house.

% Though it is natural for human beings to reason with their knowledge, it is not as easy for machines.
To help machines leverage such knowledge, many work have been done in constructing event-centric KGs \cite{zhang2020aser, zhang2022aser, sap2019atomic}.
% However, on top of that, grounding free-text to event-centric KGs is still underexplored.
The next step is to ground free-text to these KGs.
Here, work are relatively scarse.
Several characteristics of events are hindering this process:

\begin{enumerate}
\vspace{-6pt}
    \item \textit{Difficulty in representing events.} 
    First, events appear entangled in texts, meaning that they tend to share arguments with other events in the same context.
    This necessitates an event extraction step to separate events from their contexts.
    Second, when separated from the context, events lose co-reference information in the argument level.
    For instance, when viewing them out of context, it is hard to discern whether the pronoun ``they'' in event \textbf{E1} and \textbf{E2} refer to the same target.
    
    % event-related problems, extraction & normalization (e.g. interleaved events in texts, loss of coreference)
    % Events do not naturally exist in free texts. Instead, they can be interleaved and have complex relations among them:.
    % an extraction step is needed to explicitly get them. 
\vspace{-6pt}
    \item \textit{Sparsity of events.} 
    Events are sparse in natural language.
    % This is largely due to its diversity.
    For instance, one could paraphrase the event ``\textit{he is drinking a cup of dry white}'' into almost infinite new events, such as ``\textit{a person is drinking alcohol},'' or ``\textit{the general is drinking Sauvignon Blanc},'' simply by adding or removing details.
    Given the incomplete nature of event-centric KGs, matching arbitrary events to KGs has very high failure rate.
    % The sparsity comes from various descriptions of a same situation.
    % For example, by removing or adding details, one could paraphrases the situation ``\textit{he is drinking a cup of dry white}'' into almost infinite new situations, such as ``\textit{a person is drinking alcohol}'', or ``\textit{the general is drinking Sauvignon Blanc}'', which could essentially refer to the same situation.
    
    % On the other hand, the existing situational commonsense KGs may never be complete enough\cite{}.
    
    % The above characteristics of events makes it hard to exactly match (ground) natural language texts to event-centric KGs. 
    
    % (Solution: conceptualization. We tackle this by event normalization \& multi-level abstraction. Theoretical guidance: \cite{murphy2004big}.
    % Mutian's example: buying a movie ticket every time there is a new movie, we have to get the ``concept'' of buying tickets for movies so that the isolated events are linked together.)
\vspace{-6pt}
\end{enumerate}

In this work, to tackle the \textit{event representation} problem, we equip semantic parsing based event extraction (Section \ref{sec:event_extraction}) with an event normalization step (Section \ref{sec:event_normalization}), which helps separate events from contexts while preserving their arguments' co-reference information.

Motivated by human's abstract thinking process, we propose to solve the \textit{sparsity} problem by controlling the amount of details in events with a multi-level event abstraction approach (Section \ref{sec:event_abstraction}).
It conceptualizes events into multiple abstract levels by dropping argument details.
We empirically prove that these solutions largely alleviate the sparsity problem in Section \ref{sec:ablation}. 
% In practice, the event normalization step help by removing personal co-reference details.
% {\color{orange} refer to the ablation part to show the effect}

Finally, we discuss grounding the abstract events to a KG to get a joint reasoning subgraph in Section \ref{sec:event_grounding}, and present our graph neural network based prediction model in Section \ref{sec:graph_model}. 
The overall framework of our approach is shown in Figure~\ref{fig:framework}.



% In this work, we extend the retrieval-and-integration paradigm to perform high quality knowledge retrieval and interpretable reasoning on free text based narrative reasoning tasks. 
The wide adoption of AI critically needs explainability~\cite{hoffman2018metrics}. Thus, despite the appeal of a simpler pipeline (aided by the availability of large PLMs), this work focus on improving retrieval-and-integration approach.
For high quality knowledge retrieval, we propose an event acquisition pipeline including event extraction, normalization, and abstraction to mine multi-granularity events from input free texts with the help of semantic parsing.
With the acquired multi-granularity events, we use semantic matching models to ground the events to relevant eventualities in KGs, and thus construct a joint subgraph containing both events from input texts and the eventualities from KGs.
Then, we encode the subgraph with graph neural networks (GNNs) to make prediction. 
The constructed subgraph as well as the GNN parameters can provide interpretable evidence.
% Note that we still leverage PLMs for text embedding, but they are constrained in interpretable prediction, thus not used to compute the subgraph probability.
% As a result, our approach doesn't critically rely on large PLMs.

We conduct experiments on four narrative reasoning tasks and the results show that our approach can achieve stable performance gain over strong baseline models on all the tasks.
A qualitative case study show that our approach can provide human-interpretable evidence for the predictions.
The contribution of this paper is summarized as follows:

1. To our best knowledge, we are the first to propose a systematic approach to ground free texts to eventuality knowledge graphs.

2. We introduce a GNN model to perform narrative reasoning on our constructed joint subgraph.

3. Experimental results show that our approach outperforms strong baselines and achieves SOTA performance on several datasets.

4. The qualitative case study shows that our approach can provide human-interpretable evidence in narrative reasoning.



